An adaptive fractional state links circuit mechanisms to cortical dynamics across the visual hierarchy

Cortical circuits must respond flexibly to new inputs while integrating information about the past, yet the way in which neural activity reconciles these competing demands remains unclear. Combining Neuropixels recordings from six mouse visual areas with mechanistic circuit modeling, we identify a dynamical regime in which heavy-tailed superdiffusive fluctuations coexist with long-range temporal dependence and oscillations. We formalize this regime as the adaptive fractional (AF) state, using an effective mean-field theory in which spatial and temporal fractional derivatives capture heavy-tailed excursions and long-range memory, respectively. We find that dynamical exponents characterizing the AF state vary systematically across the visual hierarchy: higher visual areas exhibit weaker superdiffusion and stronger temporal memory. In the circuit model, this hierarchical shift emerges from a progressive weakening of effective inhibition. These findings extend the classical hierarchy of timescales to a hierarchy of dynamical regimes and suggest that the AF state allows cortical areas to jointly express rapid responses and long-term temporal integration.

==> main_xr_labels.tex <==
% Auto-generated by scripts/process_submission from main.aux
% Keep only label definitions needed by xr/xr-hyper cross-document refs.
\relax
\newlabel{FirstPage}{{}{1}{}{section*.1}{}}
\newlabel{FirstPage@cref}{{}{[1][1][]1}{}{}{}}
\newlabel{sec:introduction}{{I}{2}{Introduction}{section.1}{}}
\newlabel{sec:introduction@cref}{{[section][1][]I}{[1][2][]2}{}{}{}}
\newlabel{sec:effective_theory}{{II\,C}{7}{A minimal effective theory links superdiffusion, memory, and oscillations}{subsection.2.3}{}}
\newlabel{sec:effective_theory@cref}{{[subsection][3][2]II\,C}{[1][7][]7}{}{}{}}
\newlabel{eq:bifractional_neural_sampling}{{1}{7}{A minimal effective theory links superdiffusion, memory, and oscillations}{equation.1}{}}
\newlabel{eq:bifractional_neural_sampling@cref}{{[equation][1][]1}{[1][7][]7}{}{}{}}
\newlabel{eq:bfns_limits}{{2}{8}{A minimal effective theory links superdiffusion, memory, and oscillations}{equation.2}{}}
\newlabel{eq:bfns_limits@cref}{{[equation][2][]2}{[1][8][]8}{}{}{}}
\newlabel{sec:hierarchical_variation}{{II\,E}{10}{Working regimes vary systematically across the visual hierarchy}{subsection.2.5}{}}
\newlabel{sec:hierarchical_variation@cref}{{[subsection][5][2]II\,E}{[1][10][]10}{}{}{}}
\newlabel{sec:discussion}{{III}{13}{Discussion}{section.3}{}}
\newlabel{sec:discussion@cref}{{[section][3][]III}{[1][12][]13}{}{}{}}
\newlabel{subfig:schematic_experiment}{{1a}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:schematic_experiment@cref}{{[subfigure][1][1]1a}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:schematic_experiment}{{a}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:schematic_experiment@cref}{{[subfigure][1][1]1a}{[1][17][]17}{}{}{}}
\newlabel{subfig:brain_trace}{{1b}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:brain_trace@cref}{{[subfigure][2][1]1b}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:brain_trace}{{b}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:brain_trace@cref}{{[subfigure][2][1]1b}{[1][17][]17}{}{}{}}
\newlabel{subfig:lfp_increments}{{1c}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:lfp_increments@cref}{{[subfigure][3][1]1c}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:lfp_increments}{{c}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:lfp_increments@cref}{{[subfigure][3][1]1c}{[1][17][]17}{}{}{}}
\newlabel{subfig:schematic_circuit}{{1d}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:schematic_circuit@cref}{{[subfigure][4][1]1d}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:schematic_circuit}{{d}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:schematic_circuit@cref}{{[subfigure][4][1]1d}{[1][17][]17}{}{}{}}
\newlabel{subfig:membrane_potential}{{1e}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:membrane_potential@cref}{{[subfigure][5][1]1e}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:membrane_potential}{{e}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:membrane_potential@cref}{{[subfigure][5][1]1e}{[1][17][]17}{}{}{}}
\newlabel{subfig:input_current}{{1e}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:input_current@cref}{{[subfigure][5][1]1e}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:input_current}{{e}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:input_current@cref}{{[subfigure][5][1]1e}{[1][17][]17}{}{}{}}
\newlabel{subfig:potential_distribution}{{1f}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:potential_distribution@cref}{{[subfigure][6][1]1f}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:potential_distribution}{{f}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:potential_distribution@cref}{{[subfigure][6][1]1f}{[1][17][]17}{}{}{}}
\newlabel{subfig:input_distribution}{{1g}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:input_distribution@cref}{{[subfigure][7][1]1g}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:input_distribution}{{g}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:input_distribution@cref}{{[subfigure][7][1]1g}{[1][17][]17}{}{}{}}
\newlabel{subfig:empirical_mad}{{1h}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:empirical_mad@cref}{{[subfigure][8][1]1h}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:empirical_mad}{{h}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:empirical_mad@cref}{{[subfigure][8][1]1h}{[1][17][]17}{}{}{}}
\newlabel{subfig:empirical_psd}{{1i}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:empirical_psd@cref}{{[subfigure][9][1]1i}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:empirical_psd}{{i}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:empirical_psd@cref}{{[subfigure][9][1]1i}{[1][17][]17}{}{}{}}
\newlabel{subfig:empirical_fano_factor}{{1j}{17}{Figures}{figure.caption.3}{}}
\newlabel{subfig:empirical_fano_factor@cref}{{[subfigure][10][1]1j}{[1][17][]17}{}{}{}}
\newlabel{sub@subfig:empirical_fano_factor}{{j}{17}{Figures}{figure.caption.3}{}}
\newlabel{sub@subfig:empirical_fano_factor@cref}{{[subfigure][10][1]1j}{[1][17][]17}{}{}{}}
\newlabel{fig:experimental_data}{{1}{18}{\newsubref {subfig:lfp_increments} Distribution of LFP increments pooled across layer 2/3 channels (blue), each channel standardized by its own standard deviation, against a Gaussian (dashed black) and a phase-randomized (FT) surrogate that preserves each channel's power spectrum but enforces Gaussian increments (thin gray line). The annotated $\kappa $ is the median across sessions of the median excess kurtosis over channels; the surrogate value is indistinguishable from zero, so the heavy tails are not explained by the linear correlation structure. \newsubref {subfig:schematic_circuit} Snapshot of the input current in the circuit model, showing a localized activity pattern that wanders across space. The pattern's center-of-mass trajectory over the preceding window is shown as a colored line, and the dashed circle marks the neuronal patch analyzed in \subref {subfig:membrane_potential}. \newsubref {subfig:membrane_potential} Membrane potential of the excitatory neuron at the center of the patch in \subref {subfig:schematic_circuit} (upper), the spike raster of the surrounding patch population (middle), and the same neuron's synaptic input current, showing large, `bumpy' fluctuations (lower). The threshold and reset potentials are marked by solid and dashed red horizontal lines, respectively, the mean potential by a dashed gray line, and the neuron's median firing rate $\nu $ is annotated. \newsubref {subfig:potential_distribution} Distribution of membrane potentials across all excitatory neurons in the circuit model, showing a mean significantly below the spiking threshold. \newsubref {subfig:input_distribution} Step-size distribution for the synaptic input currents across all excitatory neurons in the circuit model, shown on log-log axes to highlight heavy, near-power-law tails. \newsubref {subfig:empirical_mad} Mean absolute deviation (MAD) of LFP fluctuations in layer 2/3 of the primary visual area (\texttt {VISp}, spontaneous activity; blue) and synaptic input currents in the circuit model (red), both showing a superdiffusive component with diffusion exponent $>0.5$ at short time lags. Dashed lines show power-law fits to the drawn median curves over the fitted band, with the diffusion exponent $a$ annotated; the curves are normalized in log-log coordinates, so only their slopes are comparable. For experimental data, the solid line and shaded band indicate the across-session median and IQR of within-session median values. \newsubref {subfig:empirical_psd} Power spectral density (PSD) of LFP fluctuations in \texttt {VISp} (blue) and synaptic input currents in the circuit model (red), both showing a broadband component with spectral exponent $>-2$, indicating long-range temporal dependence, alongside $\theta $ and $\gamma $ oscillatory peaks (at approximately \SI {7}{\hertz } and \SI {55}{\hertz } in the LFP). Dashed lines show the aperiodic components of a MAPPLE fit to each drawn curve, with the high-frequency exponent annotated. \newsubref {subfig:empirical_fano_factor} Fano factor of neuronal spikes in layer 2/3 of \texttt {VISp} (blue) and excitatory neurons in the circuit model (red), both showing super-Poissonian values ($>1$) and power-law scaling over intermediate time windows. Dashed lines, offset to the left for visibility, mark the scaling band fitted to each curve, and the variability exponent $c$ of each fit is annotated. The experimental fit spans only the windows drawn here, up to \SI {1}{\second }. The per-session fits quoted in the text extend to windows of \SI {10}{\second }, over which the rise of the Fano factor slows, and so give a smaller exponent (\nameref {sec:methods})}{figure.caption.4}{}}
\newlabel{fig:experimental_data@cref}{{[figure][1][]1}{[1][17][]18}{}{}{}}
\newlabel{subfig:space_fractional_drift}{{2a}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:space_fractional_drift@cref}{{[subfigure][1][2]2a}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:space_fractional_drift}{{a}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:space_fractional_drift@cref}{{[subfigure][1][2]2a}{[1][17][]19}{}{}{}}
\newlabel{subfig:space_fractional_diffusion}{{2b}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:space_fractional_diffusion@cref}{{[subfigure][2][2]2b}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:space_fractional_diffusion}{{b}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:space_fractional_diffusion@cref}{{[subfigure][2][2]2b}{[1][17][]19}{}{}{}}
\newlabel{subfig:time_fractional_drift}{{2c}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:time_fractional_drift@cref}{{[subfigure][3][2]2c}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:time_fractional_drift}{{c}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:time_fractional_drift@cref}{{[subfigure][3][2]2c}{[1][17][]19}{}{}{}}
\newlabel{subfig:time_fractional_diffusion}{{2d}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:time_fractional_diffusion@cref}{{[subfigure][4][2]2d}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:time_fractional_diffusion}{{d}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:time_fractional_diffusion@cref}{{[subfigure][4][2]2d}{[1][17][]19}{}{}{}}
\newlabel{subfig:bFNS_traces}{{2e}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:bFNS_traces@cref}{{[subfigure][5][2]2e}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:bFNS_traces}{{e}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:bFNS_traces@cref}{{[subfigure][5][2]2e}{[1][17][]19}{}{}{}}
\newlabel{subfig:diffusion_exponent}{{2f}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:diffusion_exponent@cref}{{[subfigure][6][2]2f}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:diffusion_exponent}{{f}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:diffusion_exponent@cref}{{[subfigure][6][2]2f}{[1][17][]19}{}{}{}}
\newlabel{subfig:spectral_exponent}{{2g}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:spectral_exponent@cref}{{[subfigure][7][2]2g}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:spectral_exponent}{{g}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:spectral_exponent@cref}{{[subfigure][7][2]2g}{[1][17][]19}{}{}{}}
\newlabel{subfig:diffusion_exponent_sweep}{{2h}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:diffusion_exponent_sweep@cref}{{[subfigure][8][2]2h}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:diffusion_exponent_sweep}{{h}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:diffusion_exponent_sweep@cref}{{[subfigure][8][2]2h}{[1][17][]19}{}{}{}}
\newlabel{subfig:spectral_exponent_sweep}{{2i}{19}{Figures}{figure.caption.5}{}}
\newlabel{subfig:spectral_exponent_sweep@cref}{{[subfigure][9][2]2i}{[1][17][]19}{}{}{}}
\newlabel{sub@subfig:spectral_exponent_sweep}{{i}{19}{Figures}{figure.caption.5}{}}
\newlabel{sub@subfig:spectral_exponent_sweep@cref}{{[subfigure][9][2]2i}{[1][17][]19}{}{}{}}
\newlabel{fig:theoretical_model}{{2}{20}{\newsubref {subfig:time_fractional_drift} The fractional temporal derivative turns exponential relaxation ($\beta = 1$; blue) into power-law relaxation ($\beta = 0.5$; red) via a power-law memory kernel. \newsubref {subfig:time_fractional_diffusion} The fractional temporal derivative correlates the driving fluctuations in time, lifting the unconfined power spectrum above the $f^{-2}$ scaling of normal diffusion ($\beta = 1$; blue) toward shallower slopes ($\beta = 0.5$; red). \newsubref {subfig:bFNS_traces} Sample time series showing the influence of each bFNS component: normal diffusion, L\'evy superdiffusion ($\alpha < 2$), long-range temporal correlations (LRTCs; $\beta < 1$), and oscillations ($\gamma > 0$), with parameters annotated. \newsubref {subfig:diffusion_exponent} Mean absolute deviation (MAD) of the bFNS model with $\alpha = 1.5$, $\beta = 0.85$, $\gamma = 0.03$, and $\eta = 0.01$, on a flat, unconfined potential (blue) and a unimodal potential (green). The unconfined process is superdiffusive across time lags, with its fitted diffusion exponent $a$ annotated (dashed red); the confined process is superdiffusive at short lags before flattening under confinement. \newsubref {subfig:spectral_exponent} Power spectral density (PSD) of the same processes, with the fitted spectral exponent $b$ of the unconfined process annotated (dashed red); the confined process shows a peaked spectrum with a power-law high-frequency tail, reflecting local oscillations. \newsubref {subfig:diffusion_exponent_sweep} Diffusion exponent $a$ of the unconfined bFNS model across spatial fractional order $\alpha $ and temporal fractional order $\beta $. Gray marks invalid parameter combinations, for which the self-similarity exponent lies outside $(0, 1)$; the black dashed line marks the $a = 0.5$ boundary, and the green dot the parameter combination used in \subref {subfig:diffusion_exponent} and \subref {subfig:spectral_exponent}. \newsubref {subfig:spectral_exponent_sweep} Spectral exponent $b$ across $\alpha $ and $\beta $, with the same markings}{figure.caption.6}{}}
\newlabel{fig:theoretical_model@cref}{{[figure][2][]2}{[1][17][]20}{}{}{}}
\newlabel{subfig:mean_field_schematic}{{3a}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:mean_field_schematic@cref}{{[subfigure][1][3]3a}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:mean_field_schematic}{{a}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:mean_field_schematic@cref}{{[subfigure][1][3]3a}{[1][19][]21}{}{}{}}
\newlabel{subfig:membrane_potential_mean_field}{{3b}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:membrane_potential_mean_field@cref}{{[subfigure][2][3]3b}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:membrane_potential_mean_field}{{b}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:membrane_potential_mean_field@cref}{{[subfigure][2][3]3b}{[1][19][]21}{}{}{}}
\newlabel{subfig:potential_distribution_mean_field}{{3c}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:potential_distribution_mean_field@cref}{{[subfigure][3][3]3c}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:potential_distribution_mean_field}{{c}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:potential_distribution_mean_field@cref}{{[subfigure][3][3]3c}{[1][19][]21}{}{}{}}
\newlabel{subfig:input_current_mean_field}{{3d}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:input_current_mean_field@cref}{{[subfigure][4][3]3d}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:input_current_mean_field}{{d}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:input_current_mean_field@cref}{{[subfigure][4][3]3d}{[1][19][]21}{}{}{}}
\newlabel{subfig:input_distribution_mean_field}{{3e}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:input_distribution_mean_field@cref}{{[subfigure][5][3]3e}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:input_distribution_mean_field}{{e}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:input_distribution_mean_field@cref}{{[subfigure][5][3]3e}{[1][19][]21}{}{}{}}
\newlabel{subfig:firing_rate_mean_field}{{3f}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:firing_rate_mean_field@cref}{{[subfigure][6][3]3f}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:firing_rate_mean_field}{{f}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:firing_rate_mean_field@cref}{{[subfigure][6][3]3f}{[1][19][]21}{}{}{}}
\newlabel{subfig:fano_factor_mean_field}{{3g}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:fano_factor_mean_field@cref}{{[subfigure][7][3]3g}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:fano_factor_mean_field}{{g}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:fano_factor_mean_field@cref}{{[subfigure][7][3]3g}{[1][19][]21}{}{}{}}
\newlabel{subfig:variability_exponent_mean_field}{{3h}{21}{Figures}{figure.caption.7}{}}
\newlabel{subfig:variability_exponent_mean_field@cref}{{[subfigure][8][3]3h}{[1][19][]21}{}{}{}}
\newlabel{sub@subfig:variability_exponent_mean_field}{{h}{21}{Figures}{figure.caption.7}{}}
\newlabel{sub@subfig:variability_exponent_mean_field@cref}{{[subfigure][8][3]3h}{[1][19][]21}{}{}{}}
\newlabel{fig:mean_field}{{3}{21}{An empirical bi-fractional mean field reproduces the adaptive fractional state. \newsubref {subfig:mean_field_schematic} Schematic of our mean-field construction, where a given neuron receives inputs from the surrounding network that can be approximated by the bFNS model. \newsubref {subfig:membrane_potential_mean_field} Example membrane potential trace for a simulated mean-field neuron driven by the bFNS model ($\alpha = 1.5$, $\beta = 0.8$, $\eta = 0.03$, $\gamma = 0.01$) with a target density fit from the circuit model. The threshold and reset potentials are marked by solid and dashed red horizontal lines, respectively. The mean potential is marked as a dashed gray line, and the median firing rate $\nu $ is annotated (cf.\ \cref {subfig:membrane_potential,subfig:potential_distribution,subfig:input_distribution} for the circuit model). \newsubref {subfig:potential_distribution_mean_field} The distribution of the membrane potential process shown in \subref {subfig:membrane_potential_mean_field}, showing a mean significantly below the spiking threshold. \newsubref {subfig:input_current_mean_field} Example mean-field input current trace, generated here by direct simulation of the bFNS model. \newsubref {subfig:input_distribution_mean_field} Step-size distribution for the mean-field input current process, shown on log-log axes to highlight power-law tails. \newsubref {subfig:firing_rate_mean_field} Firing rate of the mean-field neuron across spatial fractional order $\alpha $ and temporal fractional order $\beta $ (median across $10$ repeated simulations). Gray marks invalid parameter combinations, for which the self-similarity exponent lies outside $(0, 1)$. \newsubref {subfig:fano_factor_mean_field} Fano factor curves for mean-field neurons in three different regimes about the default parameters used for \subref {subfig:membrane_potential_mean_field}: i) no momentum ($\gamma = 0$; blue); ii) moderate momentum ($\gamma = 0.01$; red); and iii) no long-range memory or momentum ($\beta = 1.0$, $\gamma = 0$; green). \newsubref {subfig:variability_exponent_mean_field} Variability exponent $c$ (the exponent of the scaling regime of the Fano factor curve; see \nameref {sec:methods}) across $\alpha $ and $\beta $ for the default parameters, with the same gray masking as \subref {subfig:firing_rate_mean_field}. The color scale is clipped to $[0, 0.6]$; values fall below zero near $\beta = 1$}{figure.caption.7}{}}
\newlabel{fig:mean_field@cref}{{[figure][3][]3}{[1][19][]21}{}{}{}}
\newlabel{subfig:cortex_map}{{4a}{22}{Figures}{figure.caption.8}{}}
\newlabel{subfig:cortex_map@cref}{{[subfigure][1][4]4a}{[1][21][]22}{}{}{}}
\newlabel{sub@subfig:cortex_map}{{a}{22}{Figures}{figure.caption.8}{}}
\newlabel{sub@subfig:cortex_map@cref}{{[subfigure][1][4]4a}{[1][21][]22}{}{}{}}
\newlabel{subfig:hierarchy_l23}{{4b}{22}{Figures}{figure.caption.8}{}}
\newlabel{subfig:hierarchy_l23@cref}{{[subfigure][2][4]4b}{[1][21][]22}{}{}{}}
\newlabel{sub@subfig:hierarchy_l23}{{b}{22}{Figures}{figure.caption.8}{}}
\newlabel{sub@subfig:hierarchy_l23@cref}{{[subfigure][2][4]4b}{[1][21][]22}{}{}{}}
\newlabel{subfig:hierarchy_correlation}{{4c}{22}{Figures}{figure.caption.8}{}}
\newlabel{subfig:hierarchy_correlation@cref}{{[subfigure][3][4]4c}{[1][21][]22}{}{}{}}
\newlabel{sub@subfig:hierarchy_correlation}{{c}{22}{Figures}{figure.caption.8}{}}
\newlabel{sub@subfig:hierarchy_correlation@cref}{{[subfigure][3][4]4c}{[1][21][]22}{}{}{}}
\newlabel{subfig:circuit_diffusion_map}{{4d}{22}{Figures}{figure.caption.8}{}}
\newlabel{subfig:circuit_diffusion_map@cref}{{[subfigure][4][4]4d}{[1][21][]22}{}{}{}}
\newlabel{sub@subfig:circuit_diffusion_map}{{d}{22}{Figures}{figure.caption.8}{}}
\newlabel{sub@subfig:circuit_diffusion_map@cref}{{[subfigure][4][4]4d}{[1][21][]22}{}{}{}}
\newlabel{subfig:circuit_spectral_map}{{4e}{22}{Figures}{figure.caption.8}{}}
\newlabel{subfig:circuit_spectral_map@cref}{{[subfigure][5][4]4e}{[1][21][]22}{}{}{}}
\newlabel{sub@subfig:circuit_spectral_map}{{e}{22}{Figures}{figure.caption.8}{}}
\newlabel{sub@subfig:circuit_spectral_map@cref}{{[subfigure][5][4]4e}{[1][21][]22}{}{}{}}
\newlabel{fig:hierarchical_variation}{{4}{22}{Working regimes vary systematically across the visual hierarchy. \newsubref {subfig:cortex_map} Schematic map of the six visual cortical areas (\texttt {VISp}, \texttt {VISl}, \texttt {VISrl}, \texttt {VISal}, \texttt {VISpm}, \texttt {VISam}), colored by their anatomical hierarchy score~\cite {Harris2019d,Siegle2021} from lower (dark) to higher (light) areas. \newsubref {subfig:hierarchy_l23} Diffusion exponent $a$ and spectral exponent $b$ plotted across the six visual areas in layer 2/3 during spontaneous activity, with each area colored as in \subref {subfig:cortex_map}. Points give the across-session bootstrap median, with bars showing the 95\% confidence interval. Arrows indicate the direction in which each model parameter displaces the exponents, as that parameter is increased: the bFNS spatial fractional order $\alpha $ and temporal fractional order $\beta $, and the circuit-model synaptic I:E ratio $\delta $ and excitatory adaptation strength $\Delta g_K$, each labeled in the panel. Arrow lengths are normalized. \newsubref {subfig:hierarchy_correlation} Correlation between the dynamical exponents and the cortical hierarchy, by cortical layer. Markers show the across-session median Kendall's $\tau $ for the diffusion exponent $a$ (blue), the spectral exponent $b$ (red), and the variability exponent $c$ (teal), with bars showing 95\% percentile bootstrap intervals over $10^4$ resamples of sessions and faint points showing the per-session values behind each median. Filled markers indicate a Benjamini--Hochberg-adjusted permutation $p < 0.01$. The correlations of $a$ and $b$ are strongest in layer 2/3, where the diffusion exponent decreases and the spectral exponent increases with hierarchy score, while the correlation of $c$ is positive at every layer and significant in all but layer 4. \newsubref {subfig:circuit_diffusion_map} Diffusion exponent $a$ of the circuit model plotted against the synaptic inhibition-to-excitation ratio $\delta $, with one curve for each of five excitatory adaptation strengths $\Delta g_K$. The diffusion exponent saturates near $0.64$ at high $\delta $ (strong inhibition). As $\delta $ is lowered through the AF regime, the diffusion exponent decreases below $0.5$ during the transition to the excitation-dominated regime. \newsubref {subfig:circuit_spectral_map} Spectral exponent $b$ plotted against $\delta $ for the same values of $\Delta g_K$}{figure.caption.8}{}}
\newlabel{fig:hierarchical_variation@cref}{{[figure][4][]4}{[1][21][]22}{}{}{}}
\newlabel{tab:params}{{I}{23}{Default circuit-model parameters}{table.caption.9}{}}
\newlabel{tab:params@cref}{{[table][1][]I}{[1][23][]23}{}{}{}}
\newlabel{sec:methods}{{XI}{24}{Methods}{section.11}{}}
\newlabel{sec:methods@cref}{{[section][11][]XI}{[1][24][]24}{}{}{}}
\newlabel{subsec:experimental_data}{{XI\,A}{24}{Experimental data}{subsection.11.1}{}}
\newlabel{subsec:experimental_data@cref}{{[subsection][1][11]XI\,A}{[1][24][]24}{}{}{}}
\newlabel{subsec:circuit_sweeps}{{XI\,C}{27}{Circuit parameter sweeps}{subsection.11.3}{}}
\newlabel{subsec:circuit_sweeps@cref}{{[subsection][3][11]XI\,C}{[1][27][]27}{}{}{}}
\newlabel{sec:theoretical_model_sup}{{XI\,D}{28}{Theoretical model}{subsection.11.4}{}}
\newlabel{sec:theoretical_model_sup@cref}{{[subsection][4][11]XI\,D}{[1][28][]28}{}{}{}}
\newlabel{eq:bifractional_neural_sampling_sup}{{15}{28}{Theoretical model}{equation.15}{}}
\newlabel{eq:bifractional_neural_sampling_sup@cref}{{[equation][15][]15}{[1][28][]28}{}{}{}}
\newlabel{eq:caputo_derivative}{{16}{29}{Theoretical model}{equation.16}{}}
\newlabel{eq:caputo_derivative@cref}{{[equation][16][]16}{[1][29][]29}{}{}{}}
\newlabel{eq:effective_potential_gradient_sup}{{17}{29}{Theoretical model}{equation.17}{}}
\newlabel{eq:effective_potential_gradient_sup@cref}{{[equation][17][]17}{[1][29][]29}{}{}{}}
\newlabel{eq:riesz_derivative}{{18}{29}{Theoretical model}{equation.18}{}}
\newlabel{eq:riesz_derivative@cref}{{[equation][18][]18}{[1][29][]29}{}{}{}}
\newlabel{sec:bfns_implementation}{{XI\,E}{29}{bFNS implementation}{subsection.11.5}{}}
\newlabel{sec:bfns_implementation@cref}{{[subsection][5][11]XI\,E}{[1][29][]29}{}{}{}}
\newlabel{subsec:mean_field_model_sup}{{XI\,F}{32}{Empirical mean field}{subsection.11.6}{}}
\newlabel{subsec:mean_field_model_sup@cref}{{[subsection][6][11]XI\,F}{[1][32][]32}{}{}{}}
\newlabel{eq:mean_field_neuron}{{25}{32}{Empirical mean field}{equation.25}{}}
\newlabel{eq:mean_field_neuron@cref}{{[equation][25][]25}{[1][32][]32}{}{}{}}
\newlabel{subsec:fitting_exponents}{{XI\,G}{32}{Fitting dynamical exponents}{subsection.11.7}{}}
\newlabel{subsec:fitting_exponents@cref}{{[subsection][7][11]XI\,G}{[1][32][]32}{}{}{}}
\newlabel{subsec:hierarchical_correlation}{{XI\,H}{36}{Hierarchical correlation analysis}{subsection.11.8}{}}
\newlabel{subsec:hierarchical_correlation@cref}{{[subsection][8][11]XI\,H}{[1][36][]36}{}{}{}}
\newlabel{LastBibItem}{{83}{41}{Hierarchical correlation analysis}{section*.10}{}}
\newlabel{LastBibItem@cref}{{[subsection][8][11]XI\,H}{[1][41][]41}{}{}{}}
\newlabel{LastPage}{{}{41}{}{}{}}

